Glance to Count: Learning to Rank with Anchors for Weakly-supervised Crowd Counting

Crowd image is arguably one of the most laborious data to annotate. In this paper, we devote to reduce the massive demand of densely labeled crowd data, and propose a novel weakly-supervised setting, in which we leverage the binary ranking of two images with high-contrast crowd counts as training guidance. To enable training under this new setting, we convert the crowd count regression problem to a ranking potential prediction problem. In particular, we tailor a Siamese Ranking Network that predicts the potential scores of two images indicating the ordering of the counts. Hence, the ultimate goal is to assign appropriate potentials for all the crowd images to ensure their orderings obey the ranking labels. On the other hand, potentials reveal the relative crowd sizes but cannot yield an exact crowd count. We resolve this problem by introducing "anchors" during the inference stage. Concretely, anchors are a few images with count labels used for referencing the corresponding counts from potential scores by a simple linear mapping function. We conduct extensive experiments to study various combinations of supervision, and we show that the proposed method outperforms existing weakly-supervised methods without additional labeling effort by a large margin.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> commands.tex <==
\usepackage{amsmath}
\usepackage{nicefrac}
\usepackage{xcolor}
%\usepackage{subcaption}
\usepackage[inline]{enumitem}
%\usepackage[labelfont=bf]{caption}
\usepackage{tabularx}

% spacing
%\setlength\abovecaptionskip
%\setlength\belowcaptionskip{-6pt} % 10pt

% colors
\definecolor{colorbrewer0}{RGB}{45,45,45}
\definecolor{colorbrewer1}{RGB}{228,26,28}
\definecolor{colorbrewer2}{RGB}{55,126,184}
\definecolor{colorbrewer3}{RGB}{77,175,74}
\definecolor{colorbrewer4}{RGB}{152,78,163}
\definecolor{colorbrewer5}{RGB}{255,127,0}
\definecolor{colorbrewer6}{RGB}{255,255,51}
\definecolor{colorbrewer7}{RGB}{166,86,40}
\definecolor{colorbrewer8}{RGB}{247,129,191}
\definecolor{colorbrewer9}{RGB}{153,153,153}

\newcommand{\Perp}{\perp\!\!\! \perp}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bhy}{\hat{\mathbf{y}}}
\newcommand{\bty}{\tilde{\mathbf{y}}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\eye}{\mathbf{I}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bm}{\mathbf{m}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bhh}{\hat{\mathbf{h}}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\mR}{\mathbb{R}}
\newcommand{\mN}{\mathbb{N}}
\newcommand{\mL}{\mathbb{L}}
\newcommand{\mF}{\mathbb{F}}
\newcommand{\mE}{\mathbb{E}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cZ}{\mathcal{Z}}
\def\bgamma{\boldsymbol\gamma}

\newcommand{\figref}[1]{\Fig~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\defref}[1]{Def.~\ref{#1}}
%\renewcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\eqnref}[1]{Eq.~\eqref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}

\def\eg{e.g\onedot} \def\Eg{E.g\onedot}
\def\ie{i.e\onedot} \def\Ie{I.e\onedot}
\def\cf{cf\onedot} \def\Cf{Cf\onedot}
\def\etc{etc\onedot} \def\vs{vs\onedot}
\def\wrt{wrt\onedot}
\def\dof{d.o.f\onedot}
\def\Fig{Fig\onedot} \def\Eqn{Eqn\onedot} \def\Sec{Sec\onedot} \def\Alg{Alg\onedot}
\makeatother

% comments
\newcommand{\myparagraph}[1]{\vspace{3pt}\noindent{\bf #1}}
%\newcommand{\myparagraph}[1]{\vspace{3pt}{\bf #1}~}

==> sec_abstract.tex <==
\begin{abstract}
	\vspace{-5mm}
	Crowd image is arguably one of the most laborious data to annotate. In this paper, we devote to reduce the massive demand of densely labeled crowd data, and propose a novel weakly-supervised setting, in which we leverage the binary ranking of two images with high-contrast crowd counts as training guidance. To enable training under this new setting, we convert the crowd count regression problem to a ranking potential prediction problem. In particular, we tailor a Siamese Ranking Network that predicts the potential scores of two images indicating the ordering of the counts. Hence, the ultimate goal is to assign appropriate potentials for all the crowd images to ensure their orderings obey the ranking labels. On the other hand, potentials reveal the relative crowd sizes but cannot yield an exact crowd count. We resolve this problem by introducing ``anchors'' during the inference stage. Concretely, anchors are a few images with count labels used for referencing the corresponding counts from potential scores by a simple linear mapping function. We conduct extensive experiments to study various combinations of supervision, and we show that the proposed method outperforms existing weakly-supervised methods without additional labeling effort by a large margin.
	\keywords{Crowd Counting, Weakly-supervised Learning, Ranking}
\end{abstract} 

==> sec_main.tex <==
\vspace{-2mm}\section{Proposed Method}\label{sec:method}\vspace{-2mm}
\subsection{Problem Formulation}
%Before elaborating on the proposed method, we first briefly present the problem notations. We are

Given a set of crowd images $X = \{x_1, x_2, ... ,x_n\}$, where $x_i$ is the sample of crowd images, and $x_i \in \mathbb{R}^{H \times W \times C}$, where $H$, $W$ and $C$ denote the height, width, and number of channels respectively, our goal is to predict the object count $y_i$ of a crowd image $x_i$.
The existing works achieve the goal by learning a mapping function $M: X \rightarrow Y$ to predict the labels, \ie, $Y=\{y_1, y_2, ... , y_n\}$. Different from the previous practice, we utilize \textit{ranking labels} for supervision instead of count labels. Count labels refer to the object number of crowd images, while ranking labels are binary (i.e. $\{-1, 1\}$), each of which indicates the size relationship between the counts of two crowd images.
%and indicates precedence with respect to the counting outcome, as the relative quantity between two samples.

%We formulate the task of counting based on ranking labeled data as a ranking problem.
Formally, the crowd dataset $X$ can be expanded as a set $P$ of ranking labeled pairs. Each element of the ranking pair set $P$ in the crowd dataset $X$ is denoted as a tuple $\langle x_i, x_j, q_{i,j} \rangle, 1 \le i ~\textless~ j \le n$, where the binary ranking label $q \in \{-1,1\}$. When the crowd counts of $x_i$ and $x_j$ are subject to $y_i \gg y_j$, their size relationship can be easily identified, which means that the crowd image $x_i$ ranks higher than $x_j$, so that the corresponding label $q_{i,j}$ is set to $1$ and vice versa.

\rll{In favor of learning the ranking relationship among a set of crowd images, we introduce the \textit{crowd counting potential} $v$ that is positively correlated with the actual crowd count $y$. Thus, the goal is to learn an estimating function $f(x;w)$ to predict the potentials $v$ for all the crowd images with ranking labels, which aims to ensure the ordering of the assigned potentials obey the ranking labels. After that, the estimation function can be further used to predict the potential for any query image and the anchoring mechanism can map its potential to the absolute crowd count.}
%The ranking label for supervision could propagate the ranking signal from a pair of potential scores to mapping function weights $w$.

\begin{figure*}[t]
	\centering
	\vskip -0.25cm
	\includegraphics[width=\textwidth]{./figs/2_overview.pdf}
	\vskip -7px
	\vspace{-2mm}\caption{{Our framework consists of three stages. (1) Constructing a DAG to detect transitive relation amongst crowd images, i.e., automatic labeling, which establishes a crowd dataset with ranking labels. (2) Training the Siamese Ranking Network on ranking labels to minimize the ranking hinge loss and predict potentials (e.g. $v_1,v_2$) for crowd images, where the parameter $\mathcal{M}$ denotes the margin of the loss. (3) On the inference stage, the count of a crowd image $\hat{x}$ can be estimated by mapping the predicted potential $\hat{v}$ to actual crowd count $\hat{y}$.}}\vspace{-2mm}
	\label{fig:architecture}
\end{figure*}

\vspace{-2mm}
\subsection{Labeling Ranking Pairs}

%When training the proposed task, comparison labels are demand and each one can be produced at a glance.
For a pair of unlabeled crowd images $\{x_1, x_2\}$, if it is observed that the crowd number $y_1$ is definitely much greater than $y_2$, the ranking label $q_{i,j}$ is set to $1$, and vice versa.
%or if $y_2$ is much greater than $y_1$, $q_{i,j}$ is $0$.
If the relationship is hard to identify, no label will be added to the ranking pair set $P$.
Regarding various crowd scenarios, there are different strategies to label ranking pairs.

First, we can exploit the images from public benchmarks to train our model.
For most existing crowd counting benchmarks (\eg, ShanghaiTech \cite{zhang2016single}, UCF-QNRF \cite{idrees2018composition}), they can provide the dense annotations of object locations for crowd images and the count labels can thus be acquired without effort, which means we can easily convert them into ranking labels.
Generally, for crowd dataset $X$, the size of all ranking pairs $|P_{all}|$ is $O(n^2)$ (where $n$ is the size of dataset), in which any two images could be formed as a ranking pair. However, the number of ranking labels is much less than $n^2$, since we are only allowed to manually label the obviously distinguishable pairs of crowd images. In addition, considering that the ranking relationship is transitive, if the ranking labels, $\langle x_A, x_B, 1\rangle$ (i.e. $y_A > y_B$) and $\langle x_B, x_C, 1 \rangle$ (i.e. $y_B > y_C$), already exist in the annotated set, then $\langle x_A, x_C, 1\rangle$ or $\langle x_C, x_A, -1\rangle$ will be automatically added to the annotated set as shown in Fig.~\ref{fig:architecture}. Particularly, automatic labeling can be realized by detecting the connectivity in a directed acyclic graph, $G = (V, E)$. In specific, $V$ denotes the set of vertices, which includes all the images that occurred in the ranking pairs. $E$ denotes the set of arcs, where $\langle x_i, x_j, q_{i,j}\rangle, q_{i,j}=1$ refers to an arc $i \rightarrow j$ from the vertex $i$ to th vertex $j$ on the graph $G$ .

Nevertheless, the crowd images from public benchmarks are not sufficient to cover a large variety of scenes, so we also annotate the crowd images in the wild, so as to increase the diversity of the training data and thus strengthen the model generalizability. Thus, we attempt to collect as many unlabeled crowd images as possible. On the other hand, we restrict each collected unlabeled image to be ranked for a few times only. Actually, in practice, most of the collected images will be ranked for once, so that our crowd counting model can focus more on unseen images.

\vspace{-2mm}
\subsection{Pairwise Ranking Model}
%With the above problem definition, nextly we introduce the architecture we adopted in this work, shown in Fig.~\ref{fig:architecture} as an overview.
Our proposed Siamese ranking network architecture is illustrated in Fig.~\ref{fig:architecture}.
In specific, we employ a deep Siamese Network \cite{chopra2005learning} as the ranking model for pairwise crowd images, which is consisted of two branches of networks that share weights. The input of our model is a ranking pair $\{x_1, x_2\}$ from the set $P$. Each branch of the networks is fed with one of the image pair and outputs the corresponding potentials $v_1$ and $v_2$. We leverage a convolutional neural network (CNN) based crowd counting architecture, CSRNet \cite{li2018csrnet}, as the backbone of the Siamese network. The backbone is composed of a pre-trained CNN as the frontend for 2D feature extraction and a dilated convolutional layer for enlarging the reception fields on the backend.
%The structure can bring promising performance to congestion scene tasks.

To supervise the ranking labels, we propose to associate the predicted potentials of two network branches with the corresponding ranking labels.
Inspired by Ranking Support Vector Machine \cite{herbrich2000large}, we can train the network by minimizing the ranking hinge loss as follows:
\begin{align}
\mathcal{L} &= \sum_{x_i,x_j}max(0, f(x_j; w) - f(x_i; w) - \mathcal{M}),\nonumber\\
&\text{s.t. }	 \langle x_i, x_j, 1\rangle \text{ or } \langle x_j, x_i, -1\rangle \in P,
\end{align}
where $\mathcal{M}$ is a hyper-parameter that indicates \rll{a margin to maintain the potential difference between paired images} and $w$ refers to the network weights.

\rll{Specifically, during training, we want the model to discard the redundant samples that are easy to discriminate and cannot contribute to the model optimization.
	%	, which is always discriminated correctly and can not work on the loss.
	To do so, we set a \textit{hard sample filter} which requires the potentials $v_i$ and $v_j$, inferred from $\{x_i,x_j\}$, should be subject to the condition $\frac{v_i}{v_j} < \xi$ (or $\frac{v_j}{v_i} < \xi$), where $\xi$ is a predefined threshold to determine if the ranking labels should be abandoned.}

\vspace{-2mm}
\subsection{Anchoring Mechanism}
\rll{During inference, for any query crowd image $\hat{x}$, its predicted potential can be used to regress its crowd count. Thus, it is intuitive to compare the potential $\hat{v}$ of the query image (i.e., $\hat{v} = f(\hat{x})$) against a set of exemplar crowd images with their ground-truth counts known. }
%	Then, we can estimate the approximate range of crowd count adopting the idea of binary search. However, relying on pairwise comparison will suffer from severe error once an outlier sample appears in these ``known'' images.

\rll{In particular, we introduce a counting anchoring mechanism. We denote the labeled exemplar images as \textit{counting anchor set}. The anchor set includes a set of crowd images sampled from the training set, and their counts are specifically annotated and distributed over a large counting range, \eg, 30 $\sim$ 3,000. Thus, we can estimate the scaling mapping function $S:v \rightarrow y$ that projects the predicted potentials of the images in the anchor set to crowd counts via linear regression, as shown in Fig.~\ref{fig:architecture} \ding{174}.}

%This mapping function is not hard to be fitted from these labeled ``known'' image samples. By doing so, the queried count can be directly estimated by scaling the network output. Here these ``known'' images are called benchmark. The benchmark set is composed of a series of crowd images which the crowd numbers spread from few to more, \eg, 30 $\sim$ 3,000. The images in set could be collected arbitrarily, but they would better appears in the training set. Because the network has seen these crucial samples can avoid some bad results from outlier benchmark images as possible.

\vspace{-2mm}
\subsection{\rll{Ranking v.s. Regression}}
The reasons of choosing ranking-based scheme over regression-based methods are two fold. First, comparing to the point-based annotation, ranking labels are much easier to obtain, i.e., annotators only need to label ``close'', ``less than'', and ``greater than'' for any two crowd images. Second, ranking problem is simpler to solve than regression-based methods, because ranking relationship are invariant to any image-level geometrical transformation, which can thus improve the model robustness. On the contrary, optimizing regression model is difficult and tends to stuck with local-minima.
%\rll{Estimating ranking relationships between image pairs has several advantages over the regression metric estimation for crowd counting. Firstly, humans are better at judging relative amount. The ranking labels have a simple, discrete three way, corresponding to the ``close'', ``less than'', and ``greater than'' relationships. Thus label annotation is easier. On the other hand, ranking solves a simpler problem than metric regression. Ranking relationships are invariant to monotonic transformations of the crowd image, thereby improving the robustness of the system and providing additional qualitatively information. Training in combination with ranking would lead to much higher accuracy and faster convergence. In contrast, only training a regression network suffers from unsatisfactory local solutions and slow convergence. Therefore, instead of a count label regresser, ranking is preferred for weakly-supervised crowd counting.}
%Compared with the original count-label based regression methods, the proposed ranking method can achieve better performance with less supervision. Yet, the theoretical upperbound of the optimization objective is easy to approach. Since it seems that simply learning a good ranking model is insufficient for counting task, and a suboptimal regression model can also give perfect ranking \rll{by task definition}. But a model with perfect ranking performance may yield poor regression performance. Thus, it is a trade-off for choosing ranking or regression. \rll{Converting regression problem into ranking gives up on directly optimizing the minimum count error, but focus on the next better thing, acquiring a fast solution to the indirect ranking task and inferring the count number finally. }
However, although it is easy to obtain optimal solution for the ranking based formulation, it may not always be optimal for crowd counting. Because, the theoretical upperbound of the optimization objective when ranking is easy to approach. It seems that simply learning a good ranking model is insufficient for counting task, and a suboptimal regression model can also give perfect ranking. But a model with perfect ranking performance may yield poor regression performance.
%Converting regression problem into ranking gives up on directly optimizing the minimum count error, but focus on the next better thing, acquiring a fast solution to the indirect ranking task and inferring the count number finally.


Therefore, it is a trade-off for choosing ranking or regression. To further improve our model we propose to integrate regression and ranking-based schemes. To this end, crowd counting can be achieved in such a hybrid weakly-supervised setting. The optimization objective is consisted of two terms, i.e., pairwise ranking loss $L_{rank}(P; w)$ and regression loss $L_{reg}(D; w)$. In each iteration during training, there will be a crowd image randomly selected from $D$ and a ranking pair randomly selected from $P$ as network input. Formally, the hybrid optimization loss is defined as below:
\begin{align}
\mathcal{L}^{++} = \min_{w} \mathcal{L}_{rank}(P; w) + \alpha \mathcal{L}_{reg}(D; w),
\end{align}
where $D$ is the dataset including crowd images with count label for regression, and the parameter $\alpha$ trades off between pairwise ranking loss and regression loss. Note that, with more crowd labels used in regression, the performance benefited from regression is greater.
To make full use of the supervision from counting anchor set, we can utilize these few anchor samples with count labels as $D$ for regression.
%That can ensure a free way to combine ranking with regression.
In the most extreme case, we can attach all the training images with count labels for optimizing the regression loss term, so that it transforms our formulation into a count-label based optimization completely. Yet, with the involvement of the ranking loss term, the performance is significantly superior to the pure regression-based methods.
%Although the employed labels are exactly the same as those of naive regression method on count label, the performance is significantly improved because of the proposed ranking strategy. 
